Generative Subgraph Retrieval for Knowledge Graph-Grounded Dialog Generation

Knowledge graph-grounded dialog generation requires retrieving a dialog-relevant subgraph from the given knowledge base graph and integrating it with the dialog history. Previous works typically represent the graph using an external encoder, such as graph neural networks, and retrieve relevant triplets based on the similarity between single-vector representations of triplets and the dialog history. However, these external encoders fail to leverage the rich knowledge of pretrained language models, and the retrieval process is also suboptimal due to the information bottleneck caused by the single-vector abstraction of the dialog history. In this work, we propose Dialog generation with Generative Subgraph Retrieval (DialogGSR), which retrieves relevant knowledge subgraphs by directly generating their token sequences on top of language models. For effective generative subgraph retrieval, we introduce two key methods: (i) structure-aware knowledge graph linearization with self-supervised graph-specific tokens and (ii) graph-constrained decoding utilizing graph structural proximity-based entity informativeness scores for valid and relevant generative retrieval. DialogGSR achieves state-of-the-art performance in knowledge graph-grounded dialog generation, as demonstrated on OpenDialKG and KOMODIS datasets.

==> 3_Methods/3_3_knowledge_path_selection.tex <==
% \label{sec:3.3}

We present a Knowledge Path Retriever to obtain context-relevant knowledge paths from all possible knowledge paths motivated by \cite{lewis2020retrieval,kang2022knowledge}.
Given a dialog history $\TokenSeq$ and knowledge paths $\PathSet$, the knowledge path retriever computes a relevance score between the dialog history and each path and returns the most relevant $k$ knowledge paths.
Similar to the knowledge path embedding $\hb_p = \enc(\zb_p)$ in \eqref{eq:kpembed}, 
we feed the token sequences of dialog history $\TokenSeq$ into a Transformer encoder $\enc(\cdot)$ and compute the context vector $\hx$, which is \texttt{[CLS]} output vector, \ie, $\hb_x = \enc(\xb)$.
With the context embedding $\hb_x$ and the knowledge path embedding $\hb_p$, 
the context-relevance score between the dialog history $\xb$ and path $p$ is computed as:
\begin{equation}
s ( \xb, p ) = \mathbf{\sigma\left( \MLPx (h_{\TokenSeq})^\top MLP_p\left(h_p \right)\right)},
\label{eq:kpscore}
\end{equation}
where $\sigma$ is the sigmoid function, $\MLPx$ and $\MLPp$ are single-layer feed-forward networks to project embedding vectors onto a common space.\footnote{Note that we only fine-tune the feed-forward networks and freeze the dialog history encoder for the retrieval.}
Finally, based on the relevancy scores $s (\xb, p)$, the $k$ most context-relevant knowledge paths are retrieved. 
This Knowledge Path Retriever can be viewed as a path-level hard attention layer, which suppresses irrelevant paths and lets the model more focus on informative paths. More discussion with experimental results is in Section \ref{sec:analysis}.
We then retrieve informative paths $\hat{\PathSet}$ by selecting paths with the top $k$ relevance scores.

==> Figure_tex/constraints.tex <==
\begin{figure}
% \small
\centering
\includegraphics[width=0.8\linewidth]{Figures/constraints.pdf}
\caption{\textcolor{red}{[DRAFT]} An example of graph-constraints.}
\label{fig:constraints}
\end{figure}

==> Tables/qual_bak.tex <==
\begin{table*}[ht!]
\small
\centering
\resizebox{\textwidth}{!}  
{
    \begin{tabular}{llll}
        \toprule
          Dialog & Gold response & SURGE (Baseline) & DialogGSR (Ours) \\
         \midrule
         \midrule
         \begin{tabular}{@{}l@{}}
(a) Do you like Shaun White?\\
(b) I know he's an Olympic snowboarder he was funny in\\
\quad \ \ Friends With Benefits.\\
(a) Oh, I've never seen that movie, isn't Mila Kunis in it?\\ \quad \ \  I love her! \\
(b) She is. Justin Timberlake and Woody Harrelson were also \\ \quad \ \ in it. Shaun just played a small part. \\
(a) Do you by any chance remember who Mila Kunis is married \\
\quad \ \ too, I totally forgot.\\
\end{tabular}
& 
         \begin{tabular}{@{}l@{}}
She's married to \\ Ashton Kutcher.
\end{tabular} & 
         \begin{tabular}{@{}l@{}}
Mila Kunis is married \\ to Jennifer Lawrence.
\end{tabular} &
\begin{tabular}{@{}l@{}}
Mila Kunis is married \\ to Ashton Kutcher.
\end{tabular}\\         
    \midrule
        \multicolumn{4}{l}{\textit{\textbf{Knowledge triplets $\tau$ retrieved by Baseline}}} \\
        % & \multicolumn{3}{l}{\textit{\textbf{Knowledge triplets $\tau$ retrieved from GSR}}} \\
        \multicolumn{4}{l}{$\langle$ `Justin Timberlake', `place musical career began', `Shelby Forest' $\rangle$} \\
        % & \multicolumn{3}{l}{$\langle$ `Ashton Kutcher', `romantic relationship (with celebrities)', `Mila Kunis' $\rangle$}\\
        \multicolumn{4}{l}{$\langle$ `Justin Timberlake', `place musical career began', `Millington' $\rangle$} \\
        % \multicolumn{3}{l}{$\langle$ `\colorbox{red}{Becca Fitzpatrick}', `write', `\colorbox{yellow}{Silence}'  $\rangle$}\\
        \multicolumn{4}{l}{$\langle$ `Justin Timberlake', `romantic relationship (with celebrities)', `Scarlett Johansson'$ \rangle$} \\
        % \multicolumn{3}{l}{$\langle$ `\colorbox{yellow}{Silence}', `\colorbox{green}{released year}', `\colorbox{cyan}{2012}' $\rangle$}\\
        \midrule
        \multicolumn{4}{l}{\textit{\textbf{Knowledge triplets $\tau$ retrieved by DialogGSR~(ours)}}}\\
        \multicolumn{4}{l}{$\langle$ `Ashton Kutcher', `romantic relationship (with celebrities)', `Mila Kunis' $\rangle$}\\
        \multicolumn{4}{l}{$\langle$ `Friends with Benefits', `starred\_actors', `Mila Kunis'  $\rangle$}\\
        \multicolumn{4}{l}{$\langle$ `Friends with Benefits', `starred\_actors', `Patricia Clarkson' $\rangle$}\\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
\caption{Comparison on responses generated by SURGE~(Baseline) and DialogGSR given a dialog.}
\label{tab:qual}
\vspace{-13pt}
\end{table*}
